Deep Clustering with Measure Propagation

Deep models have improved state-of-the-art for both supervised and unsupervised learning. For example, deep embedded clustering (DEC) has greatly improved the unsupervised clustering performance, by using stacked autoencoders for representation learning. However, one weakness of deep modeling is that the local neighborhood structure in the original space is not necessarily preserved in the latent space. To preserve local geometry, various methods have been proposed in the supervised and semi-supervised learning literature (e.g., spectral clustering and label propagation) using graph Laplacian regularization. In this paper, we combine the strength of deep representation learning with measure propagation (MP), a KL-divergence based graph regularization method originally used in the semi-supervised scenario. The main assumption of MP is that if two data points are close in the original space, they are likely to belong to the same class, measured by KL-divergence of class membership distribution. By taking the same assumption in the unsupervised learning scenario, we propose our Deep Embedded Clustering Aided by Measure Propagation (DECAMP) model. We evaluate DECAMP on short text clustering tasks. On three public datasets, DECAMP performs competitively with other state-of-the-art baselines, including baselines using additional data to generate word embeddings used in the clustering process. As an example, on the Stackoverflow dataset, DECAMP achieved a clustering accuracy of 79%, which is about 5% higher than all existing baselines. These empirical results suggest that DECAMP is a very effective method for unsupervised learning.

==> Suggestions <==
From Michael:
Abstract
“improved the unsupervised clustering performance” —> “improved unsupervised clustering performance”
2 Introduction
“such as image and text” —> “such as images and text”
“Precisely due to this reason” —> “Precisely for this reason”
“As local structure preserving” —> “As local structure preservation”
“KL divergence of class membership distribution” —> “KL divergence of the class membership distribution”
“preserve local structure of the data” —> “preserve the local structure of the data”
“a special case of our algorithms” —> “a special case of our algorithm”
Section 4:
Para 1:
“to apply deep models” —> “applying deep models”
Section 8.1:
Should we give some examples of what the short texts looks like in each domain?
Section 9:
“admitting end-to-end training” —> “which supports end-to-end training”






From Qiming:
* Title: Deep Embedded Clustering Aided with Measure Propogation for Short Text Analysis
Section 2:
* Refs in 2nd paragraph, DEC, IDEC, VaDE, VAE, etc..
*“while in the original DEC...”  --> “while the decoder is discarded during clustering in DEC.”
* Contribution summarization:
-3. we provide a theoretical justificaiton for the empirical choice of the target distribution in DEC, derived from a special case of DECAMP.
-4. we propose a novel optimization procedure to address the balacing cnstraint issue in DEC, which enables effective end-to-end mini-batch training.
Section 4:
* DEC workflow summarization:
1. Initialize $\theta$ in the deep network via autoencoder pretraining and K-means clustering and obtain initial cluster predictivve distribution $q_{ik}(\theta)$ in (1)
2. With $q_{ik}(\theta)$, generate pseudo labels $p_{ik}$ according to (3)
3. With $p_{ik}$, update $\theta$ by optimizating (2) and obtain new cluster predictive distribution With $q_{ik}(\theta)$ with updated $\theta$
4. Repeat steps 2 and 3 until convergence.
Section 5:
* after (4), introduce all notations in “where”, including regularization hyperparameters

Qiming Huang  15 hours ago
Section 6:
* Since no analytic solution exits for $\theta$ and $p$ in optimizing Equation (4), we take an Alternative Minimization approach [REF] and optimize $theta$ and $p$ alternatively.  Here, we give a detailed description of this approach in solving (4).
6.1 Optimizing $p$ in pseudo label generation, given $\theta$
…
6.2 Optimizing $\theta$ in deep network, given $p$
…
* DECAMP workflow summarization would need to be modified accordingly as in the DEC workflow summarization in Section 4



